RedStone: Curating General, Code, Math, and QA Data for Large Language Models

Pre-training Large Language Models (LLMs) on high-quality, meticulously curated datasets is widely recognized as critical for enhancing their performance and generalization capabilities. This study explores the untapped potential of Common Crawl as a comprehensive and flexible resource for pre-training LLMs, addressing both general-purpose language understanding and specialized domain knowledge. We introduce RedStone, an innovative and scalable pipeline engineered to extract and process data from Common Crawl, facilitating the creation of extensive and varied pre-training datasets. Unlike traditional datasets, which often require expensive curation and domain-specific expertise, RedStone leverages the breadth of Common Crawl to deliver datasets tailored to a wide array of domains. In this work, we exemplify its capability by constructing pre-training datasets across multiple fields, including general language understanding, code, mathematics, and question-answering tasks. The flexibility of RedStone allows for easy adaptation to other specialized domains, significantly lowering the barrier to creating valuable domain-specific datasets. Our findings demonstrate that Common Crawl, when harnessed through effective pipelines like RedStone, can serve as a rich, renewable source of pre-training data, unlocking new avenues for domain adaptation and knowledge discovery in LLMs. This work also underscores the importance of innovative data acquisition strategies and highlights the role of web-scale data as a powerful resource in the continued evolution of LLMs. RedStone code and data samples will be publicly available at \url{https://aka.ms/redstone}.

==> chapters/contributions.tex <==
\section*{Contributions}
The contributors are listed in the \textbf{alphabetical order by last names}:


Yaoyao CHANG, Lei CUI, Li DONG, Shaohan HUANG, Yangyu HUANG, Yupan HUANG, Scarlett LI, Tengchao LV, Shuming MA, Qinzheng SUN, Wenhui WANG, Furu WEI, Ying XIN, Mao YANG, Qiufeng YIN, Xingxing ZHANG.




















==> chapters/discussion.tex <==
\section{Discussion}
During the construction of a general domain dataset, we have identified several key findings that can guide the creation of high-quality large-scale datasets from web data. These findings primarily involve main content extraction, document filtering, and deduplication. main content extraction sets the upper limit on dataset quality, while document filtering can significantly enhance data quality, approaching this upper limit. Deduplication can substantially reduce the dataset size, allowing models to encounter a more diverse range of data within the same number of training steps.

\subsection{Enhancements in main content Extractors Can Significantly Improve Data Quality}
\begin{table*}[t!]
  \centering
  \scriptsize
  \begin{tabular}{lrccccccccc}
  \toprule
    Method    & ARC-c  & ARC-e  & HellaSwag & OpenBookQA & PIQA & Winogrande & AVERAGE\\
  \midrule
  Paragraph Deduplication$_{shard}$ & 0.2005 & 0.3670 & 0.3364 & 0.1980 & 0.6273 & \textbf{0.5280} & 0.3762  \\
  Paragraph Deduplication$_{snapshot}$ & 0.2090 & 0.4087 & \textbf{0.3382} & 0.1740 & 0.6333 & 0.5036 & 0.3778  \\
  Trafilatura             & \textbf{0.2125} & \textbf{0.4369} & 0.3380 & \textbf{0.2100} & \textbf{0.6491} & 0.5264 & \textbf{0.3955}  \\
  \bottomrule
  \end{tabular}
  \caption{
  \textbf{Comparison on Common Sense Reasoning Tasks for Different Text Extraction Methods. The \emph{shard} indicates that paragraph-level exact deduplication is limited to within each shard, while \emph{snapshot} indicates that deduplication is limited to within each snapshot.}
  \label{tab:diss_text_extractor}
  }
\end{table*}

Currently, two main methods are employed for extracting the main content from web pages: paragraph deduplication and extractor-based main content extraction. 

\begin{itemize}
\item \textbf{Paragraph deduplication.} Introduced in CCNet, operates on the premise that non-essential content such as ``menus'' and ``login'' frequently appear across multiple pages. This method involves searching for all paragraphs on a page that also appear on other pages and removing them if they are identified as non-essential. To reduce computational cost, CCNet segments the entire web data into chunks, each limited to 5GB, and confines the deduplication search space to within these chunks, thereby isolating the main content of the page. 

\item \textbf{Extractor-based content extraction. }  Extractor analyzes the HTML elements and their content to determine if they belong to the main content. Popular tools for this method include Trafilatura, newspaper3k, and readabilipy. 
\end{itemize}

In our experiments, content extractors generally outperformed paragraph deduplication, as detailed in Table~\ref{tab:diss_text_extractor}. We identified several issues with paragraph deduplication: (1) its effectiveness is influenced by the size of the search space, (2) it cannot precisely remove noisy text, such as unique addresses or timestamps accurate to the millisecond, and (3) it may erroneously delete some relevant content. We attempted to address the search space issue by expanding it to the snapshot level, which significantly improved the scores but still fell short compared to content extractors. 

main content extractors also have their shortcomings; Trafilatura, one of the best-performing tools, has low recall and often extracts only part of the main content. Currently, no perfect content extraction tool exists for web data. 

Our results indicate that content extraction tools greatly influence data quality. In the next section, we will discuss filters, which are limited by the quality ceiling set by main content extraction tools. Therefore, developing a better content extraction tool could be a crucial direction for future research.


\subsection{A Better Filter: Enhancing Knowledge Concentration}
\begin{table*}[t!]
  \centering
  \scriptsize
  \begin{tabular}{lrccccccccc}
  \toprule
   Data & ARC-c  & ARC-e  & HellaSwag & OpenBookQA & PIQA & Winogrande & AVERAGE \\
  \midrule
  CC$_{WikiLM:30\%;KenLM:100\%}$ & 0.1971 & 0.4116 & 0.3135 & 0.1720 & 0.5930 & 0.4909 & 0.3630  \\
  CC$_{WikiLM:50\%; KenLM:100\%}$ & 0.2005 & 0.4436 & 0.3360 & 0.1800 & 0.6415 & 0.5162 & 0.3863  \\
  CC$_{WikiLM:50\%; KenLM:50\%}$ & 0.2099 & 0.4348 & 0.3345 & 0.1960 & 0.6235 & \textbf{0.5241} & 0.3871  \\
  DCLM         & 0.2159 & 0.4848 & 0.3614 & 0.1760 & 0.6615 & 0.5082 & 0.4013 \\
  FineWeb-Edu  & \textbf{0.2722} & \textbf{0.5648} & 0.3637 & 0.1940 & 0.6676 & 0.5051 & 0.4279  \\
  \ours{}-CC  & 0.2662 & 0.5181 & \textbf{0.3722} & \textbf{0.2340} & \textbf{0.6795} & 0.5162 & \textbf{0.4310}  \\
  \bottomrule
  \end{tabular}
  \caption{
  \textbf{Comparison of Common Sense Reasoning Tasks Across Different LM Filters. The Percentages in the Subscripts Indicate the Proportion of Data Retained After Filtering, Relative to the Original Dataset. And CC$_{WikiLM:50\%; KenLM:50\%}$ is Approximately Equal to the Recommended Value by CCNet.}
  \label{tab:result_of_different_lm_filters}
  }
\end{table*}

We found that the higher the concentration of knowledge in the data, the better the model performs across various tasks during testing. Other factors, such as grammar and language style, do not have a qualitative impact on data quality. For instance, text perplexity has traditionally been an important metric for measuring language quality, but it is not reliable for data quality filtering. Texts with very high perplexity can still have a positive impact. 

We first validated the n-gram-based language model filters proposed by CCNet to control text quality, including the Kneser-Ney (KenLM) filter and the WikiLM filter. In CCNet, KenLM is used to compute similarity scores between web pages and a target domain (e.g., Wikipedia). It calculates the perplexity of each text segment; lower perplexity indicates data closer to the target domain. WikiLM, introduced in LLama, assumes that web pages cited by Wikipedia are generally of higher quality, and thus trained a linear model to classify pages cited by Wikipedia versus randomly selected pages. Since the effectiveness of these filters entirely depends on the threshold settings, we experimented with different thresholds to control the proportion of retained data, as shown in Table \ref{tab:result_of_different_lm_filters}. Surprisingly, as the WikiLM filter excluded more data, the data quality actually decreased, indicating a negative impact of WikiLM on filtering. KenLM, on the other hand, performed as expected. This suggests that pages cited in Wikipedia may not necessarily be considered high-quality by the model.


FineWeb-Edu, DCLM, and \ours{} developed their own filters, all targeting the extraction of knowledge-containing data. 

\begin{itemize}
\item \textbf{FineWeb-Edu} used a Transformer-based classifier, utilizing LLama3 annotations to obtain training data for the filter, aimed at identifying educational contentt, particularly
focusing on grade-school and middle-school level knowledge.

\item \textbf{DCLM} used an n-gram-based classifier, with training data including instruction-formatted data from OpenHermes2.5 (OH-2.5) and high-scoring posts from the r/ExplainLikeImFive (ELI5) subreddit. OH-2.5 is a dataset composed of open-domain conversational data, mainly used for training and evaluating natural language processing models in dialogue generation and understanding, covering a wide range of topics from daily life to professional fields. ELI5 is a dataset from the Reddit community where users ask complex questions and receive simplified, easy-to-understand explanations, akin to explaining to a five-year-old. Such data evidently provides the model with high-density knowledge. 

\item \textbf{\ours{}} used StableLM-1.6b as a classifier, with gpt4 annotations to obtain training data for the classifier, aimed at identifying a broader range of knowledge sources, not limited to dialogues, Q\&A, or educational content.
\end{itemize}

The results in Table~\ref{tab:result_of_different_lm_filters} indicate that FineWeb-Edu, DCLM, and \ours{} can significantly improve data quality, creating a substantial gap from the raw data. Although the three methods employ different classifier structures and training data, they share a similar goal: obtaining data that contains knowledge. We believe that the pre-training objective should be to infuse as comprehensive and extensive knowledge as possible to ensure the model fully understands the real world.

\subsection{Expanding Deduplication Scope Does Not Improve Data Quality}

\begin{table*}[t!]
  \centering
  \setlength{\tabcolsep}{2pt}
  \begin{tabular}{lrccccccccc}
  \toprule
   Deduplication Scope & ARC-c  & ARC-e  & HellaSwag & OpenBookQA & PIQA & Winogrande & AVERAGE \\
  \midrule
  Snapshot-Level & 0.2466 & \textbf{0.5257} & \textbf{0.3603} & \textbf{0.2240} & \textbf{0.6681} & \textbf{0.5272} & \textbf{0.4253}  \\
  Bucket-Level & 0.2466 & 0.4760 & 0.3457 & 0.1960 & 0.6333 & 0.4917 & 0.3982 \\
  Global  & \textbf{0.2534} & 0.5164 & 0.3533 & 0.1940 & 0.6507 & \textbf{0.5272} & 0.4158  \\
  \bottomrule
  \end{tabular}
  \caption{
  \textbf{Comparison of Common Sense Reasoning Tasks Across Different Deduplication Strategies. Bucket-Level deduplication groups every 6 snapshots together for deduplication.}
  \label{tab:result_of_dedup}
  }
\end{table*}

The scope of deduplication has a significant impact on data quality, as shown in Table \ref{tab:result_of_dedup}. Contrary to our previous experience, the results indicate that narrowing the scope of deduplication yields the highest scores. This phenomenon has also been observed by FineWeb, suggesting that a smaller deduplication scale may lead to greater benefits. 

A possible explanation is that a narrower deduplication scope results in a data distribution that more closely mirrors the real world, where frequently occurring data in real life also appear multiple times in the dataset. However, we are currently unable to verify this hypothesis and will investigate it further in future work.

